A Space-Time Discontinuous Petrov-Galerkin Finite Element Formulation for a Modified Schr\"odinger Equation for Laser Pulse Propagation in Waveguides

In this article, we propose a modified nonlinear Schr\"odinger equation for modeling pulse propagation in optical waveguides. The proposed model bifurcates into a system of elliptic and hyperbolic equations depending on waveguide parameters. The proposed model leads to a stable first-order system of equations, distinguishing itself from the canonical nonlinear Schr\"odinger equation. We have employed the space-time discontinuous Petrov-Galerkin finite element method to discretize the first-order system of equations. We present a stability analysis for both the elliptic and hyperbolic systems of equations and demonstrate the stability of the proposed model through several numerical examples on space-time meshes.

==> 3_elliptic.tex <==
\section{Well-Posedness Analysis for the Elliptic Case}\label{sec: elliptic case}

Renaming $a := - \alpha > 0$, we rewrite equation~(\ref{eq:theproblem}) in the divergence form:
$$
- (a u_{,\tau} - \beta_1 u_{,\zeta})_{,\tau} 
-(- \beta_1 u_{,\tau} + u_{,\zeta} )_{\zeta} - 2 \beta_0 i u_{, \zeta} = f \, .
$$
We assume the following BCs:
\begin{description}
\item[Case]  $\zeta = 0$:   $u = u_0$.
\item[Case]  $\tau = 0$:   $u = u_0$.
\item[Case]  $\tau = T$:   $u = u_0$.
\item[Case]  $\zeta = Z$:   $- \beta_1 u_{,\tau} + u_{,\zeta} = t$.
\end{description} 
For the well-posedness analysis, it is sufficient to consider the case $u_0 = t = 0$.
Introducing the energy space:
$$
V =: \{ v \in H^1(D) \, : v =0 \text{ for } \zeta = 0 \text{ or } \tau = 0,T \}\, ,
$$
we consider the classical variational formulation:
\be
\left\{
\begin{array}{ll}
u \in V \\[8pt]
\ds \int_D (a u_{,\tau} - \beta_1 u_{,\zeta}) \bar{v}_{,\tau} + (- \beta_1 u_{,\tau} + u_{,\zeta} ) \bar{v}_{,\zeta}  - 2 \beta_0 i u_{,\zeta} \bar{v} = \int_D f \bar{v} \\[12pt]
\hfill \forall v \in V \, .
\end{array}
\right.
\label{eq:VF_2nd_order_elliptic}
\ee
The leading term is elliptic which, with the Dirichlet BCs on the three edges implies coercivity, see e.g. \cite{FE_Math_book_SIAM}, Section 2.3.1.
The first-order term represents a compact perturbation of the leading term and, therefore, the Fredholm Alternative applies, see e.g. \cite{FAbook}, Section 5.21.
In order to prove that the operator is bounded below, it is thus sufficient to demonstrate uniqueness.

Consider thus the homogeneous case $f=0$. Testing with $v=u$, we obtain
$$
\underbrace{\int_D (a u_{,\tau} - \beta_1 u_{,\zeta}) \bar{u}_{,\tau} + (- \beta_1 u_{,\tau} + u_{,\zeta} ) \bar{u}_{,\zeta}}_{\text{real number}}   - 2 \beta_0 i \int_D  u_{,\zeta} \bar{u}
= 0
$$
Focusing on the second term,
$$
\begin{array}{ll}
\ds i \int_D (\Re u_{, \zeta} + i \Im u_{,\zeta} )(\Re u - i \Im u)
& \ds = i  \int_D  \half [ ( \Re u )^2 + (\Im u )^2 ]_{, \zeta}  + \int_D \Re u_{, \zeta} \Im u - \Im u _{,\zeta} \Re u \\[12pt]
& \ds = \underbrace{i \int_0^T   \half [ ( \Re u )^2 + (\Im u )^2 ] \, d \tau}_{\text{imaginary number}} +  \underbrace{\int_D \Re u_{, \zeta} \Im u - \Im u _{,\zeta} \Re u }_{\text{real number}} \, .
\end{array}
$$
Setting the imaginary part of the left-hand side to zero, we obtain that $u = 0$ on the top boundary.
But, at the same time $ \beta_1 u_{,\tau} + u_{,\zeta} = 0$ there which implies that $u_{,\zeta} = 0$ along the top boundary as well.
We can extend thus the solution $u$ with zero to a larger domain, say  $(0,T) \times (0, 2Z)$. But the solution to the elliptic problem with constant coefficient
is analytic and, therefore, $u$ must be zero in the whole domain.
The uniqueness of the solution follows.

Well-posedness of the second-order formulation in $V \subset H^1(D)$ implies that we can replace $f$ with a general  $l \in V^\prime$ and claim the existence
of a positive constant $C>0$ such that
$$
\Vert u \Vert_{H^1(D)} \leq  C \, \Vert l \Vert_{H^{-1}(D)} \, .
$$


\paragraph*{First-order system formulation.}
Introducing fluxes $\sigma_1, \sigma_2$, we obtain the system:
\be
\left\{
\begin{array}{rl}
\sigma_1 - a u_{,\tau} + \beta_1 u_{,\zeta} & = g_1 \\[8pt]
\sigma_2 + \beta_1 u_{,\tau} - u_{,\zeta} & = g_2 \\[8pt]
- \div \sigma - 2 \beta_0 iu_{,\zeta} & = f
\end{array}
\right.
\label{eq:elliptic_1st_order_system}
\ee
accompanied with BCs: $u = u_0$ on the vertical edges and bottom edge, and $\sigma \cdot n = t$ on the top edge. The right hand side
$g_1,g_2,f \in L^2(D)$.
We follow the arguments from  \cite{Demkowicz_15} to show that the strong formulation for the first-order system is well-posed.
Again, we consider the case with homogeneous BCs, $u_0 = t = 0$.
Let $v \in V$ be an arbitrary test function. Multiplying the first two equations with $- \bfnab \bar{v}$, the last equation with $\bar{v}$, integrating over $D$,
relaxing the last equation 
and summing it all up,  we obtain the original second-order equation for $u$
with the right-hand side equal to 
$$
l(v) := - (g, \bfnab v) + (f,v) \, .
$$
The well-posedness of the second-order problem implies then that
$$
\Vert \bfnab u \Vert \lesssim \Vert l \Vert_{V^\prime} \leq  (\Vert f \Vert + \Vert g \Vert )
$$
where $\Vert \cdot \Vert$ denotes the $L^2(D)$-norm.  Moving the terms with derivatives of $u$ to the right-hand side, and using the triangle
inequality, we obtain bounds:
$$
\Vert \sigma \Vert ,\, \Vert \div \sigma \Vert \lesssim (\Vert g \Vert + \Vert f \Vert) \, .
$$
\paragraph*{Injectivity of the adjoint operator.}
Repeating the same arguments for the adjoint problem, we can show also that the adjoint operator is injective as well.
We start by reversing the role of solution $u$ and test function $v$ in the variational formulation~(\ref{eq:VF_2nd_order_elliptic}),
\be
\left\{
\begin{array}{ll}
v \in V \\[8pt]
\ds \int_D (a v_{,\tau} - \beta_1 v_{,\zeta}) \bar{u}_{,\tau} + (- \beta_1 v_{,\tau} + v_{,\zeta} ) \bar{u}_{,\zeta}  - 2 \beta_0 i v \bar{u}_{,\zeta}  = \int_D f \bar{u} \\[12pt]
\hfill \forall u \in V \, .
\end{array}
\right.
\label{eq:adjoint_VF_2nd_order_elliptic}
\ee
The essential BCs for $v$ are the same as for $u$, but the natural BC on the top edge changes. We have now
$$
- \beta_1 v_{\, \tau} + v_{,\zeta} - 2 \beta_0 i v = 0 \, .
$$
Repeating {\em exactly the same argument} as for the original variational formulation~(\ref{eq:VF_2nd_order_elliptic}),
we show the uniqueness for $v$ from which it follows that the adjoint of the operator corresponding to the first-order system~(\ref{eq:elliptic_1st_order_system})
is injective as well.

We conclude that the strong formulation for the first-order system is well-posed.  The Closed Range argument (see \cite{Demkowicz_15} for details) implies that
the ultraweak formulation for system~(\ref{eq:elliptic_1st_order_system}) is well-posed as well.


==> 4_elliptic_code.tex <==
\newpage

\section{Coding the Elliptic Case}

We will slightly reformulate the problem in the form:
$$
\left\{
\begin{array}{rll}
A^{-1} \sigma - \bfnab u & = g \\[5pt]
\div \sigma + 2 \beta_0 i u_{,\zeta} & = f \, .
\end{array}
\right.
$$
where
$$
A = \left(
\begin{array}{cc}
\alpha & - \beta_1 \\
- \beta_1 & 1
\end{array}
\right)
\qquad
A^{-1} = \frac{1}{\alpha - \beta_1^2}
\left(
\begin{array}{cc}
1 &  \beta_1 \\
 \beta_1 & \alpha
\end{array}
\right)
\, .
$$
BCs:
\begin{itemize}
\item south, west and east edge: $u = u_0$,
\item north edge: $\sigma \cdot n = t$.
\end{itemize}

\noindent Adjoint operator:
$$
A^\ast (v,\tau) = (2 \beta_0 i v_{,\zeta} + \div \tau, - \bfnab v + A^{-1} \tau) \, .
$$

\noindent Broken UW formulation:
$$
\left\{
\begin{array}{lllll}
- 2 \beta_0 i (u,v_{,\zeta}) & - (\sigma, \bfnab v) & + 2 \beta_0 i \langle n_{\zeta} \hat{u},v \rangle + \langle \hat{\sigma} \cdot n, v \rangle & = (f,v) \qquad & v \in H^1(\Omega_h) \\[8pt]
(u, \div \tau) & + (A^{-1} \sigma, \tau) & - \langle \hat{u}, \tau \cdot n \rangle & = (g,\tau) & \tau \in H(\div, \Omega_h) 
\end{array}
\right.
$$

\newpage


==> save.tex <==


\paragraph*{Defining the boundary operator \boldmath{$M$}.}
We discuss the four faces of the computational rectangular domain in Fig.~\ref{fig:domain}.
\begin{figure}[h!]
	\centering
	\includegraphics[width=.4 \textwidth]{figures/domain.pdf}
	\caption{Domain of interest.}
	\label{fig:domain}
\end{figure}
\begin{description}
\item[Case:] $\zeta = 0$ with normal $n = (0,-1)$. We set
$$
D = - A^\zeta,\quad M := A^\zeta \, .
$$
Boundary condition  $(D - M)U  = - 2 A^\zeta  U = 0 $ is equivalent to setting initial conditions for both components $u$ and $v$.
\item[Case:] $\zeta = Z$ with normal $n = (0,1)$. We set
$$
D =  A^\zeta,\quad M := A^\zeta \, .
$$
Boundary condition  $(D - M)U  = 0 U = 0 $ is automatically satisfied and it does not imply any BCs on $u$ and $v$.
\item[Case:] $\tau = T$ with normal $n = (1,0)$, $D = A^\tau$. We compute the generalized eigenvectors:
$$
A^\tau b = \lambda A^\zeta b \, .
$$
We obtain:
$$
\begin{array}{lll}
\lambda_1 = - \beta_1 - \sqrt{\beta_0 \beta_1}  \approx -11 < 0
\qquad 
& b_1 = \frac{(- \lambda_1, 1)^T}{\sqrt{1 + \lambda_1^2}} \approx (0.996, 0.091)^T \\[12pt]
\lambda_2 = - \beta_1 + \sqrt{\beta_0 \beta_1} \approx 9 > 0
\qquad 
& b_2 = \frac{(- \lambda_2, 1)^T}{\sqrt{1 + \lambda_2^2}} \approx   (-0.994, 0.110)^T  \, .
\end{array}
$$
The unit eigenvectors $b_1,b_2$ form an orthonormal basis with respect to the weigted inner product 
$$
(U,V)_{A^\zeta} :=  V^\ast A^\zeta U \, .
$$
We have:
$$
V^\ast D U  = \lambda_1 (U,b_1)_{A^\zeta} \overline{(V,b_1)_{A^\zeta}} + \underbrace{ \lambda_2 (U,b_2)_{A^\zeta} \overline{(V,b_2)_{A^\zeta}}}_{=: V^\ast M U}  \, .
$$
Matrix $M$ is thus semi-positive definite, and setting $(D-M)U = 0$ is equivalent to specifying the inflow spectral component of $U$, as expected.
Note that
$$
(U,b_1)_{A^\zeta} \approx 0.996 u + 8.963 v
$$
and, therefore, knowing what value of $v$ should we use, is essential.
\item[Case:] $\tau = 0$ with normal $n = (-1,0)$, $D = - A^\tau$.  The eigenvalues from the previous case flip the sign.
We obtain:
$$
\begin{array}{lll}
\lambda_1 =  \beta_1 - \sqrt{\beta_0 \beta_1} \approx -9 < 0
\qquad 
& b_1 = \frac{( \lambda_1, 1)^T}{\sqrt{1 + \lambda_1^2}} \approx   (-0.994, 0.110)^T  \\[12pt] 
\lambda_2 =  \beta_1 + \sqrt{\beta_0 \beta_1}  \approx 11 > 0
\qquad 
& b_2 = \frac{(\lambda_2, 1)^T}{\sqrt{1 + \lambda_2^2}} \approx (0.996, 0.091)^T \, .
\end{array}
$$
We have:
$$
V^\ast D U  = \lambda_1 (U,b_1)_{A^\zeta} \overline{(V,b_1)_{A^\zeta}} + \underbrace{ \lambda_2 (U,b_2)_{A^\zeta} \overline{(V,b_2)_{A^\zeta}}}_{=: V^\ast M U}  \, .
$$
Matrix $M$ is thus semi-positive definite, and setting $(D-M)U = 0$ is equivalent to specifying again the inflow spectral component of $U$.
We have
$$
(U,b_1)_{A^\zeta} \approx -0.994 u + 10.932 v
$$
\end{description}
\textcolor{red}{Ankit, Judit. Please check my algebra. I am surprised that the contribution of $v$ on vertical boundaries is so large. This defies my intuition.
The good news is that I figured out (I think) how to make sense of traces. Since the coefficients are constant, the requirement that $A U \in (L^2(D))^2$
translates into that the directional derivatives of the spectral components must be in (scalar) $L^2(D)$. And we know how to handle the trace operators
for the pure convection.
}

